BeMERC: Behavior-Aware MLLM-based Framework for Multimodal Emotion Recognition in Conversation

Multimodal emotion recognition in conversation (MERC), the task of identifying the emotion label for each utterance in a conversation, is vital for developing empathetic machines. Current MLLM-based MERC studies focus mainly on capturing the speaker's textual or vocal characteristics, but ignore the significance of video-derived behavior information. Different from text and audio inputs, learning videos with rich facial expression, body language and posture, provides emotion trigger signals to the models for more accurate emotion predictions. In this paper, we propose a novel behavior-aware MLLM-based framework (BeMERC) to incorporate speaker's behaviors, including subtle facial micro-expression, body language and posture, into a vanilla MLLM-based MERC model, thereby facilitating the modeling of emotional dynamics during a conversation. Furthermore, BeMERC adopts a two-stage instruction tuning strategy to extend the model to the conversations scenario for end-to-end training of a MERC predictor. Experiments demonstrate that BeMERC achieves superior performance than the state-of-the-art methods on two benchmark datasets, and also provides a detailed discussion on the significance of video-derived behavior information in MERC.

==> table3.tex <==
%1.中心
%2.标题
%3.表宽
%4.三线表
%5.行高
%6.列宽
% \newcommand{\floatingtext}[1]{\kern-0.2em\makebox[0pt][l]{#1}}
% \newcommand{\up}[1]{\floatingtext{\scriptsize($\uparrow$#1)}}

\begin{table}[t!]
\renewcommand{\arraystretch}{1}
\setlength{\tabcolsep}{7pt}  % 调整列间距
\centering
\resizebox{1.0\linewidth}{!}
{
\begin{tabular}{l|cccccc}
\toprule
\multirow{2}{*}{Modality} &  &                                                                                                                                        
                         \multicolumn{2}{c}{IEMOCAP} &  & \multicolumn{2}{c}{MELD} \\
                         % &  & Acc.        & F1          &  & Acc.       & F1         &  & Acc.         & F1           &  & Acc.        & F1          &  & Acc.         & F1           &  & Acc.           & F1  
                          &  & Acc.           & w-F1  
                          &  & Acc.           & w-F1            \\ \midrule


T+A+V                  &  & 74.98 & 74.88       &  & 71.18 & 69.78    \\ 
\hdashline
T                 &  & 70.97 & 70.70       &  & 69.27 & 67.13    \\ 
A                 &  & 61.42 & 61.15       &  & 60.22 & 55.21    \\ 
V                 &  & 44.05 & 43.96       &  & 57.20 & 49.59    \\ 
T+A                 &  & 73.81 & 73.79       &  & 69.46 & 68.69    \\ 
T+V                 &  & 70.73 & 70.45       &  & 68.19 & 67.97    \\ 
A+V                 &  & 59.70 & 59.33       &  & 63.29 & 58.47     
% SpeechCueLLM                  &  & - & 72.6       &  & - & 72.6 

% RGAT                     &  & 90.0        & 90.0        &  & 90.0       & 90.0       &  & 90.0         & 90.0         &  & 90.0        & 90.0        &  & 90.0         & 90.0         &  & 90.0           & 90.0          &  & 90.0           & 90.0          \\ \hdashline
% LLMERC
%                 &  & 58.33        & 57.14        &  & 87.76       & 81.29       &  & 75.00         & 73.94         &  & 80.59        & 69.90       &  & 69.90         & 74.78         &  & 60.37           & 66.38          &  & 71.66           & 71.51          \\ 
% LLMERC-Beh
%                 &  & 56.94        & 59.42        &  & 88.16       & 84.54       &  & 72.66         & 75.20         &  & 70.00        & 69.39       &  & 80.27         & 79.87         &  & 73.75           & 72.70          &  & 74.98           & 74.88          
                \\ \bottomrule
\end{tabular}
}
\caption{Results of using different modalities. `T', `V' and `A' respectively refer to `Text', `Visual', and `Audio'.}
\label{tab3}
\end{table}


==> table5.tex <==
%1.中心
%2.标题
%3.表宽
%4.三线表
%5.行高
%6.列宽
% \newcommand{\floatingtext}[1]{\kern-0.2em\makebox[0pt][l]{#1}}
% \newcommand{\up}[1]{\floatingtext{\scriptsize($\uparrow$#1)}}

\begin{table}[t!]
\renewcommand{\arraystretch}{1}
\setlength{\tabcolsep}{7pt}  % 调整列间距
\centering
\resizebox{1.0\linewidth}{!}
{
\begin{tabular}{l|cccccc}
\toprule
\multirow{2}{*}{} &  &                                                                                                                                        
                         \multicolumn{2}{c}{IEMOCAP} &  & \multicolumn{2}{c}{MELD} \\
                         % &  & Acc.        & F1          &  & Acc.       & F1         &  & Acc.         & F1           &  & Acc.        & F1          &  & Acc.         & F1           &  & Acc.           & F1  
                          &  & Acc.           & w-F1  
                          &  & Acc.           & w-F1            \\ \midrule


LLMERC                  &  & 71.66 & 71.51       &  & 70.22 & 68.90    \\ 
w S+L                  &  & 73.56 & 73.33       &  & 70.23 & 69.10    \\

% w L                 &  & 74.32 & 74.20       &  & 70.31 & 69.55    \\

w M+L                 &  & 73.62 & 73.75       &  & 70.19 & 69.43    \\
% \hdashline
w S+T                 &  & 74.32 & 74.20       &  & 70.31 & 69.55    \\

% w P                  &  & 73.32 & 73.10       &  & 70.45 & 69.10    \\
% \hdashline
w M+T                  &  & 74.98 & 74.88       &  & 71.18 & 69.78    
% \hdashline
% T                 &  & 70.97 & 70.70       &  & 69.27 & 67.13    \\ 
% A                 &  & 61.42 & 61.15       &  & 60.22 & 55.21    \\ 
% V                 &  & 44.05 & 43.96       &  & 57.20 & 49.59    \\ 
% T+A                 &  & 73.81 & 73.79       &  & 69.46 & 68.69    \\ 
% T+V                 &  & 70.73 & 70.45       &  & 68.19 & 67.97    \\ 
% A+V                 &  & 59.70 & 59.33       &  & 63.29 & 58.47     
% SpeechCueLLM                  &  & - & 72.6       &  & - & 72.6 

% RGAT                     &  & 90.0        & 90.0        &  & 90.0       & 90.0       &  & 90.0         & 90.0         &  & 90.0        & 90.0        &  & 90.0         & 90.0         &  & 90.0           & 90.0          &  & 90.0           & 90.0          \\ \hdashline
% LLMERC
%                 &  & 58.33        & 57.14        &  & 87.76       & 81.29       &  & 75.00         & 73.94         &  & 80.59        & 69.90       &  & 69.90         & 74.78         &  & 60.37           & 66.38          &  & 71.66           & 71.51          \\ 
% LLMERC-Beh
%                 &  & 56.94        & 59.42        &  & 88.16       & 84.54       &  & 72.66         & 75.20         &  & 70.00        & 69.39       &  & 80.27         & 79.87         &  & 73.75           & 72.70          &  & 74.98           & 74.88          
                \\ \bottomrule
\end{tabular}
}
% \caption{}
% Results of different behavior fusion strategies. `S' refer to `directly introduce the generated behavior into the stage of emotion analysis. `T' regard behavior analysis as the
% initial stage. `M' refer to feed different types of behaviors into the large model for induction and introduce it into the initial stage.

% Results of different behavior fusion strategies. `S' refer to `directly introduce the generated behavior into the stage of emotion analysis. `M' regard behavior analysis as the
% initial stage. `L' refer to feed different types of behaviors into the large model for induction and introduce it into the initial stage. `T' refer to feed different types of behaviors into the large model for induction and introduce it into the initial stage.}
\caption{
Results of different behavior fusion strategies.`S' and  `M' represent extraction methods. `L' and  `T' represent training paradigms. `S' refers to design three different templates to extract three behavior information respectively, then summarize three behavior. `M' refers to use one template to extract facial expressions, body language, and posture together. `L' regards one-stage training. `T' regards two-stage training.}

% ‘M’ refers to directly
% introduce the generated speaker characteristics into the
% stage of emotion analysis. ‘R’ and ‘S’ regard speaker
% identification and speaker characteristics injection as the
% initial stage


% , `L' and `P' respectively refer to `facial expression', `body language' and `posture'.
% }
\label{tab5}
\end{table}

